LazyLedger: A Distributed Data Availability Ledger With Client-Side Smart Contracts

We propose LazyLedger, a design for distributed ledgers where the blockchain is optimised for solely ordering and guaranteeing the availability of transaction data. Responsibility for executing and validating transactions is shifted to only the clients that have an interest in specific transactions relating to blockchain applications that they use. As the core function of the consensus system of a distributed ledger is to order transactions and ensure their availability, consensus participants do not necessarily need to be concerned with the contents of those transactions. This reduces the problem of block verification to data availability verification, which can be achieved probabilistically with sub-linear complexity, without downloading the whole block. The amount of resources required to reach consensus can thus be minimised, as transaction validity rules can be decoupled from consensus rules. We also implement and evaluate several example LazyLedger applications, and validate that the workload of clients of specific applications does not significantly increase when the workload of other applications that use the same chain increase.

==> sections/notes.tex <==
\section{Notes/Drafts}

\subsection{Consensus}

\begin{itemize}
    \item The only consensus rule is that the data being added to the chain is available. (And a max blocksize limit.)
    \item The blockchain is purely used for ordering data, not validating data. (Proof-of-publication oracle.)
    \item Data structure: CT-style Merkle tree + Reed-Solomon encoding?
    \item Merkle tree structure where intermediate nodes are labelled with the range that their leafs start with, so that 'lighter' nodes can process only data relevant to them. Happy-case: miners correctly order the Merkle tree, things are efficient. Unhappy-case: miners don't correctly order it, security isn't violated but things are less efficient.
    \item Number of samples that need to be made should be proportional to stake of entity verifying a block.
\end{itemize}

\subsubsection{Relevant Deleted Theorem From Fraud Proofs Paper}

%
% ---BEGIN EXTRACT---
%
\begin{theorem} %\label{th:euler1785}
(Euler~\cite{euler1785}) the probability that the number of distinct elements sampled from a set of $n$ elements, after $c$ drawings with replacement of $s$ distinct elements each, is at least all but $\lambda$ elements\footnote{This problem is also known as \emph{the coupon collector's problem} with group drawing~\cite{ferrante2014coupon}.}:
\begin{eqnarray}\label{eq:pe}
p_{e}(Z \geq n-\lambda) &=& 1-\sum_{i=1}^\infty(-1)^i{\lambda+i-1\choose\lambda}{n\choose\lambda+i}\bigr(W_i\bigr)^c \\ \nonumber
\textrm{where} && W_i={n-\lambda-i\choose s}\bigg/{n\choose s}
\end{eqnarray}
\end{theorem}

\begin{theorem}%\label{th:matrix-lottery-variable}

In a $2n$-by-$2n$ extended data matrix, given a set of block producers in a shard which have varying shares of stake, a network parameter $h$ that represents the minimum fraction of honest stake in a shard to prevent a dishonest block producer from controlling the chain, and a network parameter $p$ that is the desired probability for the honest stake in a shard to have sampled all the data in another shard's chain, then the number of shares $s$ each block producer has to sample proportional to its stake $m$ must be such that the following equality is satisfied:

$\displaystyle p = 1 - \sum_{k=1}(-1)^k{(n+1)^2+k-1\choose (n+1)^2}{(2n)^2\choose (n+1)^2+k}\left[{(2n)^2-(n+1)^2-k\choose s} \bigg/ {(2n)^2\choose s}\right]^{\frac{h}{m}}$

\begin{proof}

Note that $p$ is equivalent to the formula in \Cref{theorem:matrix-lottery}, but $c = \frac{h}{m}$. This means that each block producer in the shard assumes that all of the other block producers in the shard have the same amount of stake $m$, thus for the stake to add to up to 1, there are $\frac{1}{m}$ other block producers, of which only $\frac{1}{h}$ are honest, thus there are $\frac{h}{m}$ honest block producers.

To prove that this probability remains consistent when $m$ is variable, we need to deconstruct Euler's formula in \Cref{theorem:euler-lottery}. We are concerned with the following term in Euler's formula, which denotes the probability that after $d$ drawings, exactly $k$ elements will not appear:

\begin{align*}
\displaystyle (W_t)^d&&W_t=\left[{n-\lambda-k\choose t}\bigg/{n\choose t}\right]
\end{align*}

It is assumed in Euler's formula that in all $d$ drawings, $t$ samples are made, thus $W_t$ is multiplied by itself $d$ times. However, if $t$ differs, then the probability that after $d$ drawings, exactly $k$ elements will not appear is $W_{t_1}\times W_{t_2}\times...\times W_{t_d}$, instead of $(W_t)^d$.

We thus need to prove, that given $\displaystyle w=W_{t_1}^{\frac{h}{m_1}}=W_{t_2}^{\frac{h}{m_2}}=...=W_{t_d}^{\frac{h}{m_d}}$ and $h=m_1+m_2+...+m_3$, then $w=W_{t_1}W_{t_2}...W_{t_d}$.

This can be proven as follows.

\begin{align}
w&=W_{t_1}^{\frac{h}{m_1}}\\
&=W_{t_1}^{\frac{m_1+m_2+...+m_3}{m_1}}\\
&=W_{t_1}^{\frac{m_1}{m_1}}W_{t_1}^{\frac{m_2}{m_1}}...W_{t_1}^{\frac{m_d}{m_1}}\\
&=\left[W_{t_1}^{\frac{h}{m_1}}\right]^\frac{m_1}{h}\left[W_{t_1}^{\frac{h}{m_1}}\right]^\frac{m_2}{h}...\left[W_{t_1}^{\frac{h}{m_1}}\right]^\frac{m_d}{h}\\
&=w^\frac{m_1}{h}w^\frac{m_2}{h}...w^\frac{m_d}{h}\\
&=W_{t_1}W_{t_2}...W_{t_d}
\end{align}

\end{proof}
\end{theorem}
%
% ---END EXTRACT---
%

\subsection{Client-driven Transaction Model}

\begin{itemize}
    \item The meaning and validity of all transactions is decided by clients.
    \item There would be a `core' UTXO DAG for the money system, that should be verified by block producers if they want to collect fees.
    \item There would be many `side' DAGs that read from the core DAG, but they should the core DAG should not point to them otherwise block producers would have to verify the side DAGs if they want to collect fees.
\end{itemize}

\subsection{Applications}

\begin{itemize}
    \item Applications should only read, but not write to, the core money system DAG.
    \item Domain name registration system: domains can be registered if money is sent to a certain address on the money DAG.
    \item Asset and tokens: there can be many asset/token DAGs. Smart contracts could facilitate the initial sale: e.g. sent money to this address, you get a token.
    \item Crowdfunding smart contracts?
\end{itemize}

\subsection{Implementation and Performance}

\begin{itemize}
    \item Implementation applications above.
    \item Performance analysis #1: an application only causes size of state storage to grow for clients following that applications.
    \item Performance analysis #2: an application causes CPU usage to grow significantly higher for clients following that applications, than everyone else, which should be neglible.
    \item Performance analysis #3: bandwidth growth for probabilistic blocks minimal vs simplistic blocks.
\end{itemize}

\subsection{Removed Probabilistic Validity Rule Extension}

We provide an extension of the scheme suited for \sysname to strengthen the guarantees of the scheme. In particular, the scheme is originally designed for a light client/full node paradigm, and assumes that there is a minimum number of light clients in the network such that enough samples are made to reconstruct the whole block, as discussed in \Cref{sec:data-availability}. However in \sysname all nodes are effectively `light clients' because even consensus nodes are not required to download or verify the full block data if they use the Probabilistic Validity Rule. Therefore, if there are only a few consensus nodes and not enough nodes in the network making sample requests, it is possible that the consensus algorithm used by $\mathsf{inChain}$ may return a chain that does not have data availability, causing consensus nodes to build on top of an invalid chain.

It would thus be desirable for \Cref{def:data-availability-soundness} and \Cref{def:data-availability-agreement} to hold true for consensus nodes regardless of the number of other types of nodes that there are in the network. As a fallback assumption in case there are not enough nodes, we could set a threshold for the minimum percentage of the consensus `stake' that is assumed to be honest.\footnote{In this context we use `stake' to mean a `unit' of consensus, \eg in proof-of-work this would be the percentage of hashing power, and in proof-of-stake this would be percentage of tokens staked.} Honest consensus nodes could sample a quantity of shares in the block that is proportional to the stake that they have, such that if the assumption that there is a threshold of minimum percentage of honest consensus stake holds true, then enough samples would have been made by the consensus nodes alone to reconstruct the whole block. The rational for this is that consensus nodes with more stake can afford to sample more shares per block, because their block reward would be higher or they would have more resources.

\mustafa{TODO: Clean up below--it is a very messy draft.}
\mustafa{The importance of the equation below is that it shows that it is possible to determine the figuring out the samples a node needs to make does not require that node to know the distribution of stake in the network. This is important because other nodes can lie about which parts of the stake they control; \eg a Sybil attack. It sounds counter-intuitive, but the proof is there.}

%\Cref{th:matrix-lottery-variable} shows the probability that all the consensus nodes collectively sample enough shares to reconstruct the whole block, given each node samples proportionally to how much stake they control such that.

\Cref{th:matrix-lottery-variable} shows the formula for individual consensus nodes to calculate how many shares it needs to sample to achieve a desired probability for the honest stake in the network to have sampled all the block data. Note that interestingly, to make this calculation, a consensus node only needs to know how much stake itself holds and no specific information about the other consensus nodes in the system.

\begin{theorem}\label{th:matrix-lottery-variable}
    Suppose an erasure code with $n$ shares that can tolerate up to $\lambda$ unavailable shares. Given a set of consensus nodes which have varying shares of stake, a network parameter $h$ that represents the minimum fraction of honest stake to prevent a set of dishonest consensus nodes from controlling the chain, and a network parameter $p$ that is the desired probability for the honest stake in the network to have sampled all the data in a block, then the number of shares $s$ each consensus node has to sample proportional to its stake $m$ must be such that the following equality is satisfied:
    \begin{eqnarray}
        p_{e}(Y \geq n-\lambda) &=& 1-\sum_{i=1}^\infty(-1)^i{\lambda+i-1\choose\lambda}{n\choose\lambda+i}\bigr(W_i\bigr)^\frac{h}{m} \\ \nonumber
        \textrm{where} && W_i={n-\lambda-i\choose s}\bigg/{n\choose s}
    \end{eqnarray}
\end{theorem}
\begin{proof}
    Note that $p$ is equivalent to Euler's formula in \Cref{th:euler1785}, but $c = \frac{h}{m}$. This means that each consensus node in the network assumes that all of the other consensus nodes in the network have the same amount of stake $m$, thus for the stake to add to up to 1, there are $\frac{1}{m}$ other consensus nodes, of which only $\frac{1}{h}$ are honest, thus there are $\frac{h}{m}$ honest consensus nodes.

    To prove that this probability remains consistent when $m$ is variable, we need to deconstruct Euler's formula in \Cref{th:euler1785}. We are concerned with the following term in Euler's formula, which denotes the probability that after $d$ drawings, exactly $k$ elements will not appear:

    \mustafa{TODO: Make the notation below consistent; different variables are being used.}
    \begin{align*}
        \displaystyle (W_t)^d&&W_t=\left[{n-\lambda-k\choose t}\bigg/{n\choose t}\right]
    \end{align*}

    It is assumed in Euler's formula that in all $d$ drawings, $t$ samples are made, thus $W_t$ is multiplied by itself $d$ times. However, if $t$ differs, then the probability that after $d$ drawings, exactly $k$ elements will not appear is $W_{t_1}\times W_{t_2}\times...\times W_{t_d}$, instead of $(W_t)^d$.

    We thus need to prove, that given $\displaystyle w=W_{t_1}^{\frac{h}{m_1}}=W_{t_2}^{\frac{h}{m_2}}=...=W_{t_d}^{\frac{h}{m_d}}$ and $h=m_1+m_2+...+m_3$, then $w=W_{t_1}W_{t_2}...W_{t_d}$.

    This can be proven as follows:
    \begin{align}
        w&=W_{t_1}^{\frac{h}{m_1}}\\
        &=W_{t_1}^{\frac{m_1+m_2+...+m_3}{m_1}}\\
        &=W_{t_1}^{\frac{m_1}{m_1}}W_{t_1}^{\frac{m_2}{m_1}}...W_{t_1}^{\frac{m_d}{m_1}}\\
        &=\left[W_{t_1}^{\frac{h}{m_1}}\right]^\frac{m_1}{h}\left[W_{t_1}^{\frac{h}{m_1}}\right]^\frac{m_2}{h}...\left[W_{t_1}^{\frac{h}{m_1}}\right]^\frac{m_d}{h}\\
        &=w^\frac{m_1}{h}w^\frac{m_2}{h}...w^\frac{m_d}{h}\\
        &=W_{t_1}W_{t_2}...W_{t_d}
    \end{align}
\end{proof}
